Groomed Event Shapes at HERA and the sPHENIX TPC

This thesis summarizes the work of the author in two directions, both aimed at the study of quantum chromodynamics (QCD). The first topic presented is a measurement of groomed event shapes using archived data collected by the H1 experiment at HERA. The data analysis methods and physics implications of the results are discussed, with the goal of improving the theoretical description of the hadronic final state in electron-hadron collisions before the construction of the Electron-Ion Collider (EIC). The second topic concerns the sPHENIX experiment, which is now installed at the Relativistic Heavy Ion Collider (RHIC). The sPHENIX physics program and apparatus will be discussed, along with a description of each of the subdetectors. Special attention will be dedicated to the operating principles, design, and construction of the time projection chamber (TPC).

==> sections/acknowledgements.tex <==
In nature's infinite book of secrecy \\
A little I can read.\newline

I wish to dedicate this thesis to everyone who made it possible. In particular my advisor, Tom Hemmick, whose boundless expertise and didactic abilities never cease to impress me. I thank Axel Drees and Abhay Deshpande for their wisdom and encouragement in pursuits academic and otherwise. The nuclear experiment group at Stony Brook is a singular environment. In that group, I gained the breadth of experience befitting a physicist, and I will be forever grateful to have been a part of it. I thank Peter Jacobs for teaching me the beauty of jet physics and the finer points of data analysis. I thank my many collaborators in both H1 and sPHENIX; cooperation is the cornerstone of modern science, and I am grateful to have participated in not one but two such ventures. I thank the long list of physicists who have patiently endured my questions in lectures, seminars, and coffee breaks. \newline

I need mention my dear friends, Ty, Schafer, Grant, Jack, Brandon, and Daniel. All things are impermanent, but our friendship is one of the few pillars upon which I can always rely. I thank also my friends at Stony Brook, who helped me weather the storm of graduate school. I am lucky to have benefited from the generosity of so many family members during my Ph.D., especially that of Marty, Ann, Kate, Seth, Pete, and Chris. I regret not being able to thank everyone by name, but you know who you are.\newline

An endless gratitude is owed to Lindsay and Lwaxana. Their companionship breathes life into every day. \newline

Finally, I thank my parents, who, among so much else, inspired in me the curiosity that has made studying physics such a pleasure. Words cannot express what I owe them. 


